Advances in Anti-Deception Jamming Strategies for Radar Systems: A Survey

Deception jamming has long been a significant threat to radar systems, interfering with search, acquisition, and tracking by introducing false information that diverts attention from the targets of interest. As deception strategies become more sophisticated, the vulnerability of radar systems to these attacks continues to escalate. This paper offers a comprehensive review of the evolution of anti-deception jamming techniques, starting with legacy solutions and progressing to the latest advancements. Current research is categorized into three key areas: prevention strategies, which hinder the ability of jammers to alter radar processing; detection strategies, which alert the system to deception and may classify the type of attack; and mitigation strategies, which aim to reduce or suppress the impact of jamming. Additionally, key avenues for further research are highlighted, with a particular emphasis on distributed, cognitive, and AI-enabled radar systems. We envision this paper as a gateway to the existing literature on anti-deception jamming, a critical area for safeguarding radar systems against evolving threats.

==> backup_text/background.tex <==

\section{Jamming in Radar Systems}\label{sec:jamming_in_radar}
This section introduces deception jamming strategies against radar systems. First, we present a general taxonomy of jamming attacks in~\Cref{sec:jamming_general_taxonomy}, and then set the stage for a focused discussion on radar deception jamming in~\Cref{sec:jamming_deception_taxonomy}. 


\subsection{Background on Radar Systems}

maybe here we can talk about how deception can be affected by the presence of extended targets~\cite{kong2022active}

\subsubsection{Types of Radar Systems}
\hl{I think there is no need to do a taxonomy of radar systems, because the focus is on anti-deception jamming, and we are already doing a taxonomy of jamming systems. Nevertheless, we could have some introduction explaining different radar types, emergence of distributed radar, etc.}

Non-distributed radar systems can be classified into monostatic, bistatic, and multistatic categories. Monostatic radar is the most traditional form, where the transmitter and receiver are co-located at the same site. This configuration, while simpler, is more vulnerable to deception jamming because it relies on signal reflections from a single location, making it easier for jammers to manipulate the radar's perception.
%
In contrast, bistatic radar separates the transmitter and receiver spatially. This separation allows for different perspectives on the target, increasing resilience to jamming techniques by complicating the jammer’s ability to deceive both the transmitter and receiver simultaneously.
%
Multistatic radar systems take this further by incorporating multiple transmitters or receivers operating independently. This setup offers greater spatial diversity, improving resistance to various jamming techniques. \cred{However, these systems can lack the real-time data sharing capabilities seen in more modern radar networks, such as distributed radar systems, which have emerged as a solution to improve jamming resistance and target tracking through collaborative operation. The introduction of distributed radar systems offers further advantages in terms of jamming resilience and real-time data integration, making them a focus of current research.}
%
A distributed radar system can include monostatic, bistatic, or multistatic units. The term refers to how these systems are networked and collaborate, not the specific architecture of the individual radar components.

Passive radar can be used as a standalone anti-jamming technique, leveraging external signals for detection and making it inherently less susceptible to jamming since it doesn't emit signals. It can also be combined with monostatic radar in a hybrid system, where passive radar provides additional resilience and helps detect jammers, while the monostatic radar focuses on higher-resolution detection.

\subsubsection{Tracking in Radar Systems}
\hl{Difference between tracking at signal level (range gate selection, etc.) and at data level (once detections have been obtained, e.g., target tracking)}
\cred{This subsubsection I created only because I am confused about when we use inner signal processing tracking strategies and the tracking strategies with the observations of range or position... Probably in the end whatever we write here would directly go into the State Model-Based Strategies Section...}

Book on multiple target tracking with radar applications: \cite{blackman1986multiple}

In radar systems, tracking occurs on two distinct levels: signal-level tracking and data-level tracking. At the signal level, the radar directly processes the received signals and tracks either the real target or a false target, such as one created by range deception jamming (e.g., RGPO). Here, the radar system can be tricked into locking onto the false target as it manipulates the range gate, causing the radar to lose track of the real object. On the other hand, data-level tracking involves post-detection algorithms like Multiple Hypothesis Tracking (MHT), which operate on the detections provided by the radar. MHT generates and maintains multiple hypotheses about the detections, allowing it to manage uncertainty and distinguish between real targets, false targets (from jamming), and clutter. This multi-level approach enables better decision-making by refining the radar’s potentially confused outputs through advanced data association and hypothesis management.

\subsection{General Taxonomy of Jamming} \label{sec:jamming_general_taxonomy}

\begin{figure*}
\centering
  \includegraphics[width=0.95\textwidth]{figures/class notes 4.jpeg}
  \vspace{-.05cm}
  \caption{General Taxonomy of Jamming. \cred{I am not so sure yet that RGPO/RGPI... are implemented also a stand-off jamming. Should try to find literature like that to be sure.}}
   \label{fig:intro:jamming_taxonomy}
\end{figure*}

Jamming is referred to as both electronic attack (EA) and electromagnetic countermeasures (ECM). It involves using electromagnetic signals to temporarily disrupt or neutralize enemy systems without causing physical destruction, making it a "soft kill" method. A fundamental principle of jamming is to target the receiver, not the transmitter, to prevent the receiver from processing intended signals effectively.
%
Considering~\cite[Chapter 9]{ew_101}, jamming is classified in four ways (see Figure~\ref{fig:intro:jamming_taxonomy}): by the type of signal (communications versus radar); by the way it attacks the jammed receiver (cover versus deception); by jamming geometry (self-protection versus stand-off); and by the way it protects a friendly asset (decoy versus classical jammer). We also decided to add the categorizations regarding coherence (coherent versus incoherent jamming) and cooperation (cooperative versus non-cooperative jamming). In the following subsections, we dive into each of these categorizations.
%
%
\subsubsection{Communications vs. Radar Jamming}
%
Jamming can be classified by the type of signal it targets, which can either be communications or radar. Communications jamming interferes with the ability of a receiver to recover information from its desired signal by disrupting the flow of information between communicating entities. On the other hand, radar jamming interferes with the radar's ability to recover information about a target from its return signal. This prevents radar systems from accurately detecting or tracking objects, impacting their effectiveness in locating or identifying threats. As radar and communication systems become more integrated, particularly with the rise of joint radar-communication (JRC) systems, the distinction between the two types of jamming is blurring, as JRC technologies share hardware and frequency bands, making them susceptible to both radar and communication jamming~\cite{8972666}.

%
\cred{Explain that GNSS jamming is also different because satellites are located at approx. 20e3 km from Earth and consequently received satellite signal is buried in noise so you don't need much power to overpower and cause jamming, and that typically when u mimic the GNSS signal it is called spoofing - actually: check definition of spoofing for radar systems? (I am mentioning this cause I was confused by this when starting the freedom project 1st year)} Global Navigation Satellite System (GNSS) jamming could also be included in this taxonomy. Similar to communications jamming, it disrupts the reception of signals transmitted by a source (in this case, satellites from a navigation constellation), but this time targeting positioning systems. As communications and GNSS jamming are beyond the scope of this paper, interested readers are directed to~\cite{silva2023comprehensive, radovs2024recent} for comprehensive surveys on GNSS jamming, spoofing, and their countermeasures, and to~\cite{pirayesh2022jamming} for a review of jamming attacks and anti-jamming strategies in wireless networks.

\subsubsection{Cover vs. Deception Jamming}
%
Cover jamming transmits high-power signals to overwhelm an enemy’s receiver with noise, reducing the signal-to-noise ratio (SNR) and making it difficult for the receiver to detect the true signal. When the SNR is sufficiently lowered, the receiver can no longer track or detect the target effectively. Deceptive jamming, on the other hand, manipulates the radar by inserting false signals that appear valid. This misleads the radar into tracking a false target by altering its perception of range, angle, or velocity, causing the true target to go undetected.


\subsubsection{Self-Protection vs. Stand-off Jamming}
%
Self-protection jamming originates from a jammer carried on the platform that is being detected or tracked. The goal is to directly protect the platform itself by emitting jamming signals to confuse or blind the enemy's detection systems. Stand-off jamming, on the other hand, involves a jammer located on a separate platform, transmitting jamming signals to protect another platform. In this scenario, the protected platform is typically within the lethal range of the enemy's weapons, while the stand-off jammer remains outside the lethal range, providing protection from a safe distance.


\subsubsection{Decoy vs. Classical Jamming}
A decoy is a special kind of jammer designed to appear to enemy radar as more similar to the protected platform than the platform itself. Unlike classical jammers, which interfere with the radar’s operation, a decoy does not directly disrupt radar functionality. Following~\cite[Chapter 10]{ew_101}, decoys are classified into three types: expendable, which are launched for short-term use and discarded; towed, attached by a cable to an aircraft or ship for longer protection; and independent maneuver, self-propelled decoys offering flexible movement for missions like ship protection or forward defense. These decoys serve three main purposes: to overwhelm enemy defenses with false targets (saturation), to divert attacks away from the real target (seduction), and to provoke the enemy into revealing offensive capabilities by responding to a decoy (detection).


\subsubsection{Incoherent vs. Coherent Jamming}
%%
%\shuo{Strategies or techniques or mechanism? If this is classification of strategies, maybe we can put it in the section I. C. But I also prefer to put it here. Then we need to think about the terminology here: maybe 1-7 are the taxonomy for strategy and section C is for different mechanisms.}
Coherent jamming involves precise synchronization with the radar’s signal, while incoherent jamming disrupts radar performance with unsynchronized noise or broad-spectrum interference. Examples of the latter include barrage jamming, which overwhelms the radar with wideband noise across many frequencies, spot jamming, which targets a specific frequency band to disrupt radar operations, and swept jamming, which continuously moves across a range of frequencies, causing intermittent interference and covering a broad spectrum over time without saturating all frequencies simultaneously. Incoherent jamming typically requires more power but is easier to implement, relying on brute force to overwhelm the radar. In contrast, deception jamming methods, the focus of this paper, are coherent techniques that require less power but are more sophisticated, designed to mislead radar by generating false detections. There are also coherent methods that are less sophisticated and use synchronized noise to interfere, such as Coherent Blink Jamming, which turns on and off in sync with the radar's PRI, causing intermittent interference that confuses the radar's ability to track targets.

\subsubsection{Non-Cooperative vs. Cooperative Jamming}
Non-cooperative jamming involves a single jammer acting independently to disrupt radar or communication systems, lacking coordination with other jammers. Cooperative jamming, on the other hand, is a coordinated effort among multiple jammers, allowing them to synchronize their actions and share information for more effective interference. Especially in the context of distributed radar systems, it has gained increasing relevance in recent years.
%
\cite{9032116} explores a cooperative deception technique using dual-source jamming to disrupt radar fusion by generating false angular measurements. \cite{electronics11020184} examines distributed cooperative jamming by UAV swarms, where agents coordinate to enhance jamming effectiveness.

\subsubsection{Monopulse Effective vs. Non-Monopulse Effective Jamming}
\cred{I am not sure we should add this category. We will discuss methods that use monopulse radar and that is fine. Maybe we can leave the category but mention that we do not make a selection for this one.}
%
Monopulse radars are difficult to jam, particularly in self-protection scenarios where the jammer is located on the target. These radars gather all necessary tracking information from a single pulse, making them resistant to traditional jamming techniques. In some cases, a high J/S ratio from a stand-off jammer or well-deployed decoys and chaff can be effective. However, even if range information is denied, the radar can still track by angle, making self-protection jamming especially challenging. The two main approaches to jamming monopulse radars are exploiting known radar weaknesses or manipulating the radar's angle-tracking information within a single resolution cell, with the latter being more effective.
%
The interested reader may refer to~\cite[Chapter 9.9]{electronics11020184} for a description of deceptive techniques for monostatic radar.

\cred{I did not find a category for intentional vs. unintentional jamming. I do not know if, contrary to GNSS, jamming is always malicious. Myabe because GNSS signal is low power so could even jam it without wanting to. Maybe it is worth mentioning though.}

\hl{Cognitive vs. Non-Cognitive? Check that survey about CEW}

\subsubsection{Focus of this Study (wrt General Taxonomy of Jamming)}
%
figure 2. the non highlighted ones they dont work in deception jamming as is so we do not focus on them, and the antijamming taxonomy we are describing does not apply to nonhighlighted ones\\
\hl{I think in the end we will realize most of the literature we are checking is on self-protection jamming and non-cooperative. Probably the amount of literature being otherwise will be so small that we can just mention in these subsections where we have just explained the categories so that people know they exist but definitely not the focus of our paper.}

Our primary objective is to explore anti-jamming strategies designed to counter a specific branch of jamming methods. In particular, we focus on radar jamming (category 1), deception jamming (category 2), classical jamming (category 4),  coherent techniques (category 5), and non-monopulse effective jamming (category 7). It is important to note that category 3 (self-protection vs. stand-off jamming) is not mutually exclusive. For instance, deception jamming techniques, such as RGPO, can be employed in both self-protection and stand-off scenarios, depending on the location of the platform executing the deception.
%
Additionally, we consider both cooperative and non-cooperative jamming in our analysis, although the body of literature on cooperative jamming strategies is still limited, and consequently, so is the research on countermeasures against it.
%
%When false targets are generated to mimic the dynamics of the real target, we refer to this as classic jamming with seduction decoy capabilities.
%Similarly, multiple fake targets can be classified as both classical jamming, when false signals are generated at different range gates or Doppler shifts, and decoy jamming, when these false targets are designed to mimic the dynamics of a real target.
%

\hl{Explain that we focus on main-beam jamming because...}
Systems face significant challenges from deception jammers in the main beam due to the directional nature of antennas, which can typically mitigate jamming impacts in the side lobes. These jammers can intercept radar signals and generate false targets using Digital Radio Frequency Modulated (DRFM) technology, making it challenging to detect real targets within the main beam~\cite{lan_suppression_2020}. The jammer using DRFM monitors and stores signals emitted by the radar. Mainbeam jamming can occur when the interference source is co-located with the target or positioned at the same angle and distance as the target~\cite{wang_main-beam_2020}. \cblue{(Include an explanation of the example involving two planes from~\cite{xu2015deceptive})}.

\subsection{Radar Deception Jamming Strategies}
\label{sec:jamming_deception_taxonomy}
In most cases, deception jammers rely on repeating the radar signal to mislead the radar system. Traditionally, analog techniques such as instantaneous frequency (IF) jamming and delay lines have been used. These methods manipulated the radar signal by introducing time delays or other modifications without digital processing. These analog systems, while functional, were less precise and less flexible, offering only limited control over how the signal was modified. The introduction of Digital Radio Frequency Memory (DRFM) represented a significant advancement in deception jamming. DRFM allows for precise digital capture and manipulation of the radar signal, enabling jammers to store the incoming signal, modify it with high accuracy (e.g., applying delays, Doppler shifts), and retransmit it with near-perfect fidelity. While some advanced techniques can generate new, synthetic signals without repeating the original radar signal, these are less common.

In~\cite{wang2016deceptive}, they analyze the properties of target signal and deceptive jamming in time and frequency domains and model the received signal model.

We will first introduce single-target deception jamming methods, which focus on misleading the radar about the characteristics or location of a single target. This includes attacks in the range, Doppler, amplitude and angle domains. Following this, we will explore multiple-target deception jamming techniques, which aim to confuse the radar by generating or simulating multiple false targets, overwhelming the system with misleading information.



\subsubsection{RGPO/RGPI Attacks (Range Domain)}

\hl{Explain what are RGPO attacks}

Range Gate Pull-Off (RGPO) attacks are a type of self-protection jamming strategy commonly used by systems facing radar-guided threats. These attacks exploit weaknesses in the automatic range gate tracking circuits of tracking radars (such as Target Tracking Radars or TTRs). The radar's range gate is the primary mechanism used to select and track a specific target, typically locking onto the target's return signal.

The RGPO jammer intercepts the radar's signal and retransmits it with higher power, creating what is known as a cover pulse. This cover pulse captures the radar’s range gate by tricking the radar into tracking the stronger, false return, while simultaneously causing the radar's automatic gain control (AGC) to lower its sensitivity, making the real return appear weaker. Once the jammer has control of the range gate, it begins introducing time delays into the retransmitted cover pulses. These delays cause the radar’s range gate to shift away from the real target, gradually moving to false positions.

When the range gate has shifted sufficiently far from the real target, the jammer shuts down, leaving the radar without a valid target to track. As a result, the radar is forced to restart its search, acquisition, and lock process to reacquire the target. This tactic buys critical time for the jammer's platform, allowing it to evade radar-guided threats.

Range deception jammers exploit weaknesses in the automatic range gate tracking circuit of a TTR. Cover pulses capture the range gate used for TOI selection, after which the jammer introduces time delays. 
Range gate pull-off (RGPO) is a self-protection strategy where the attacker uses cover pulses to capture the range gate used for TOI selection and adds delays to shift it away from the target. Once it has moved significantly, the jammer shuts down and the TTR is forced to restart its search~\cite{fundamentals_ew,blair_benchmark_1998}.


\cred{Should we do a taxonomy for the jamming types and do a table with the ones we have found? If so, we will have optimization methods. Or should we just classify the type of jamming being mitigated when doing the taxonomy for antijamming methods?}

\hl{There is some literature on RGPO attack optimization, explain from the perspective of the attacker the literature}
%
Efforts in the literature focus on optimizing RGPO strategies for track deception.
%
The intricate nature of jammer-radar interactions complicates quantitative optimization and leads to the exploration of black-box RGPO jamming, where the jammer lacks knowledge of the TTR tracking model~\cite{10032699, jia_intelligent_2020}, unlike in the white-box scenario~\cite{9776498}.
%

\hl{RGPI Attacks}

Range gate pull-in (RGPI) attacks are typically considered impractical~\cite{6159736} due to the assumption that the TTR employs waveform diversity and pulse agility strategies~\cite{zhang_new_2013, akhtar_eccm_2007}, including the use of random OFDM signals~\cite{schuerger2009performance}. Mitigating RGPI attacks is more manageable because the advancement of the false signal to an earlier time creates a predictable pattern, enabling radar systems to distinguish between true and false signals more effectively. More advanced techniques are required to effectively mitigate RGPO attacks. 

\subsubsection{VGPO/VGPI Attacks (Doppler Domain)}

As mentioned in~\cite{zhang_new_2013}, three types of velocity deception jamming usually appear in modern jamming techniques. Velocity gate pull off (VGPO): The VGPO jammer initially creates a false target with the same Doppler frequency as the true target. The magnitude of the false target is much higher than that of the true target and the radar receiver’s automatic gain control is forced to reduce the gain. The jammer then increases the Doppler frequency, making the target seem even farther out of the Doppler cell where the true target exists. Finally the jammer switches off, leaving the radar with a broken lock. Multiple false targets (MFT): Multiple targets are created simultaneously with different Doppler frequencies. Two blinking false targets (TBFT): In blinking jamming mode, two jammers of the same operation mode are switched on and off according to a prescribed patten or almost randomly.

~\cite{frazer2020deception} presents a jamming technique that targets Doppler Beam Sharpening (DBS) radars, often used in missile seekers for ground mapping and clutter discrimination. The proposed method generates false targets at precise locations within the radar's DBS image by delaying and adding a Doppler shift to the intercepted radar signal. The authors analyze how tracking errors, caused by incorrect estimation of the missile's trajectory, affect the positioning of the false targets.


\subsubsection{Coordinated RVGPO (Range/Doppler Domains)}

\subsubsection{Ampltiude Domain}
On Off (or swept amplitude modulation), Count Down

\subsubsection{Angle Domain}
Inverse Gain, Beam Scan Modulation (Fixed or Swept Poke up gate), Cross Eye , Cross Pol

\subsubsection{Multiple False Targets}

\cite{iqbal2020effective} introduces a self-protection jamming technique for deceiving wideband LFM (Linear Frequency Modulation) radars by generating multiple false targets.

Interrupted-Sampling Repeater Jamming (ISRJ) is used in~\cite{7858673} against linear frequency modulated (LFM) radar to generate multiple false targets by sampling and retransmitting the radar's signal at specific intervals, confusing the radar's target detection by introducing echoes at various ranges.
%
The work in~\cite{mehmood2021novel} intercepts radar signals and applies time modulation to create delayed versions of the signal, which are transmitted back to the radar to simulate false targets at varying ranges along the same direction as the real target. Simultaneously, using the null-steering capability of FDA radar, the real target is hidden by placing a null in the radar's radiation pattern at its exact range and direction, making it effectively invisible. 
%
\cite{ali2022electronic} simulates these false targets using Linear Frequency Modulated (LFM) waveform-based pulsed Doppler radar and demonstrates the effectiveness of this technique in creating single and multiple false targets.



%Both RGPO and repeater jammers involve resending the radar signal back to the radar with a delay. In both cases, the jammer interacts with the radar's signal, modifying the time it takes for the signal to return to the radar to deceive the radar system.
%Repeater jamming and RGPO both resend the radar's signal with a delay but differ in purpose. Repeater jamming creates multiple false targets by varying the delay, overwhelming the radar with targets at different ranges. In contrast, RGPO gradually increases the delay, tricking the radar into tracking a false range for a single target, ultimately causing it to lose track of the real target.  In RGPO (Range Gate Pull-Off) attacks, the goal is to gradually shift the radar’s range gate away from the true target, meaning the radar will likely detect either the real target or the false (RGPO-induced) target, but not both simultaneously. The RGPO signal replaces the true target's signal over time as it pulls the radar’s range gate away, tricking the radar into tracking the false range.


◦ Doppler: Multiple Doppler False Targets (MDFT)
◦ Range/Doppler: Multiple Range Doppler False Targets (MRDFT), Coordinated RVGPO
◦ Spoofing (coherent or not-coherent false targets)


~\cite{vehicle_target}: introduces a novel deception jamming method designed for vehicle targets in the context of continuous wave ground surveillance radar. The core contribution of the paper lies in combining both translational motion and micro-Doppler (m-D) modulation to generate false target echoes with higher fidelity, making it harder for radar systems to distinguish between real and false targets.

\subsubsection{Networked/Cooperative/Distributed (?) Jamming}
\cite{rao2020deception}: cooperative deception jamming technique using noncoherent dual-source jamming to disrupt track-to-track radar fusion systems. By leveraging a distributed radar network, the approach introduces false angular information, creating persistent angular errors that mislead the fusion process. This prevents the radar systems from correctly associating the target tracks from different radar stations, effectively impairing the system's ability to maintain accurate target tracking.


\subsubsection{Synthetic Aperture Radar (SAR) Deception Jamming (Image Reconstruction Deception)}
The ability of synthetic aperture radar (SAR) to provide all-weather, high resolution imagery has made it a popular tool for use in both military and civilian applications. Thus, one of the key areas of study in electronic countermeasures has been SAR jamming and anti-jamming research~\cite{moreira2013tutorial}.
%
\cite{shenghua2004study} discusses various methods of jamming SAR systems and explores the unique challenges posed by SAR's special features, such as high processing gain and large antenna apertures. The paper highlights that jamming SAR is more difficult than conventional radar due to SAR’s ability to focus on signals over time and space, making it more resilient to interference. he study highlights two primary jamming methods: barrage jamming, which requires significantly high power to affect SAR because of its ability to compress noise during processing, and deceptive jamming, which is more effective because it creates false targets or covers real ones, confusing the radar system. The paper concludes that combining deceptive jamming with barrage jamming can be particularly effective, as the noise and false signals together make it harder for SAR to accurately detect and image real targets.
%
Direct-path jamming and multipath jamming are the two broad categories into which SAR jamming may be divided based on electromagnetic wave propagation path characteristics~\cite{delaurentis2011multipath}. Scattered wave deception jamming in Synthetic Aperture Radar (SAR) is a technique where a jammer intercepts SAR signals, modifies them (by adjusting time-delay and phase), and retransmits these modified signals back to the radar. The goal is to create false echoes or scenes that deceive the SAR system into displaying incorrect information, effectively masking or covering the real target~\cite{tao2007study}. Efforts have been made in the literature to enlarge the jammed area~\cite{zhao2014improved}, being the balance between computational complexity and focus depth a concern. Methods such as~\cite{liu2014frequency} have been proposed to efficiently generate well-focused jamming signals while maintaining manageable computational load even in real-time operations.
%

In a similar way to the previously commented paper (\cite{mehmood2021novel}) mentioned the multiple false targets type of jamming subsection,~\cite{wang2019multi} uses the FDA antenna's unique ability to transmit signals with angle-, range-, and time-dependent beampatterns, enabling the creation of multiple false targets or scenes within SAR images. The paper explores how the number and location of these false targets can be manipulated by adjusting FDA parameters, such as the frequency offsets between array elements.

\cred{Networked jammers/multireceiver against SAR:}
%
\cite{zhou2019deception} presents a deceptive jamming technique against near-field SAR using networked jammers. The proposed method leverages multiple slave receivers that intercept SAR signals and collaborate with a master jammer to perform precise time difference of arrival (TDOA) calculations.
%
\cite{tian2016multi} proposes a multi-receiver deception jamming method against SAR. The proposed approach leverages a network of receivers to intercept SAR signals and accurately calculate motion parameters using time difference of arrival (TDOA). This enables precise modulation of the jamming signal without relying on exact radar motion parameters, which are often difficult to obtain in practice.



\subsubsection{Focus of this Study (wrt Deception Jamming Taxonomy)}
\helen{change this to start of dection}\\
\newline
In Table XXX, we provide a clear and concise summary of the deception jamming methods for which we are researching countermeasures. The table includes, for each technique, the name, classification in terms of categories 3 and 6 from the General Jamming Taxonomy, along with relevant references. 
%

Now that we have explored the various radar deception jamming techniques, we shift our focus to the radar systems themselves, as we prepare to discuss the anti-jamming strategies designed to counter these methods. The next section provides a taxonomy for strategies against radar deception jamming, detailing the techniques used to mitigate the impact of deception jammers, with particular attention to methods such as RGPO, VGPO, and multiple false targets.


==> manuscript_sections/taxonomy/draft.tex <==
\subsubsection{SAR-specific Image Reconstruction Defenses}
\shuo{find a place to put SAR, or remove it.}

\hl{Synthetic Aperture Radar (SAR)}
\cred{This should not be a new category, as methods for antideception in SAR can be encompassed in the previous categories, but I am leaving the info here so that we can think of how to distribute it (I need to read the papers carefully to be able to classify). I think that when describing jamming types we can describe in detail specific cases of SAR, monopulse radar and Doppler radar, but mention the antijamming methods are encompassed together (eitherway in the table we will say if they use sar/monopulse/doppler radar/multistatic).}

The last few years have seen the development of several efficient algorithms for deceptive jamming mitigation for SAR, which may be grouped into three categories: dynamic synthetic aperture (DSA), multichannel, and waveform diversity~ \cite{9120221}. \cred{get more references from~ \cite{9120221}}


The method in~ \cite{9120221} proposes a novel Azimuth Phase Coding (APC)-based method to suppress high-fidelity deceptive jamming in SAR, particularly focusing on scenarios involving intermittent sampling. The method leverages the APC principle, which applies azimuth phase modulation and demodulation, followed by azimuth filtering, to separate and suppress deceptive jamming signals.

 \cite{chen2024deceptive} introduces a novel slow-time Group Phase Coding (GPC) technique to suppress deceptive jamming in single-channel SAR. By dividing transmitted pulses into two groups and applying different phase codes, the method offsets the deceptive jamming signals, which aids their detection.

Pulse agility with SAR: \cite{1435879}

The method in~ \cite{wang2017high} is designed to suppress retransmission deception jamming. It proposes a high-performance anti-retransmission deception jamming method for MIMO Synthetic Aperture Radar (SAR), using Orthogonal Frequency Division Multiplexing (OFDM) Linear Frequency Modulation (LFM) signals to counteract the effects of retransmitted jamming. The method involves transmitting random phase-modulated signals through multiple channels to increase signal complexity, making it difficult for jammers to intercept and retransmit effectively. By synthesizing sub-band signals into a wideband signal, the approach improves the Signal-to-Interference Ratio (SIR) and reduces jamming effects. \cred{this is also waveform diversity, right? and MIMO...}

A body of literature focuses on evaluating the performance of deception jamming against SAR~ \cite{zhonggan2017centroid, 7893506}. An effective jamming evaluation method should not only quantify the impact of jamming on SAR imaging but also help optimize jamming techniques. Current evaluation approaches are generally classified into three categories: the information criterion, the power criterion, and the efficiency criterion~ \cite{tang2021evaluation}. \cite{tian2020performance} uses a multifeature fusion approach, combining dominant indicators such as signal-to-jamming ratio, image entropy, and structural similarity~ \cite{1284395}, with recessive indicators automatically extracted using a convolutional neural network (CNN) to assess the effectiveness of jamming.
%

==> manuscript_sections/taxonomy/prevention_table_2.tex <==
\begin{table*}[htp]
\small
\centering
\caption{Overview of prevention strategies for the suppression of radar deception jamming (see~\Cref{sec:prevention}).}\label{table:jamming_prevention}
\begin{tabular}{|c|p{0.5cm}|p{0.6cm}|p{5.3cm}|p{1.5cm}|p{4cm}|}
\hline
 \rowcolor{blue!10}
\textbf{\begin{tabular}[c]{@{}c@{}}Receiver \\ Processing \\ Approach\end{tabular}} & \multicolumn{1}{c|}{\textbf{Ref.}} & \multicolumn{1}{c|}{\textbf{Year}} & \multicolumn{1}{c|}{\textbf{Description}} & \multicolumn{1}{c|}{\textbf{Deception Domain}} & \multicolumn{1}{c|}{\textbf{Challenges}} \\ \hline
\multirow{6}{*}{\begin{tabular}[c]{@{}c@{}}Correlated \\ Processing\end{tabular}} & \cite{1435879} & 2005 & \parbox[t]{5.3cm}{Randomization of \gls{LFM} chirp parameters with a two-stage matched filter.} & \multirow{6}{*}{\parbox[t]{1.5cm}{Range-Doppler}} & \multirow{6}{*}{\parbox[t]{4cm}{Coherence breaks with agile waveforms, leading to high sidelobe patterns.\\ Highly vulnerable, cannot handle agile deception attacks.}} \\ \cline{2-5}
 & \cite{schuerger2009performance} & 2009 & \parbox[t]{5.3cm}{Randomization of \gls{OFDM} subcarrier coefficients and variation in their number.} &  &  \\ \cline{2-5}
 & \cite{zhang_new_2013} & 2013 & \multirow{3}{*}{\parbox[t]{5.3cm}{\gls{RPIP} with optimization of the initial phases aided by multi-channel processing.}} &  &  \\ \cline{2-3}
 & \cite{7131032} & 2015 &  &  &  \\ \cline{2-3}
 & \cite{7485306} & 2016 &  &  &  \\ \cline{2-5}
 & \cite{s17010123} & 2017 & \parbox[t]{5.3cm}{\gls{OFDM}-\gls{LFM} radar with randomly phase-modulated subcarriers.} &  &  \\ \hline
\multirow{5}{*}{\begin{tabular}[c]{@{}c@{}}Compressed \\ Sensing\end{tabular}} & \cite{7330288} & 2015 & \multirow{3}{*}{\parbox[t]{5.3cm}{\gls{RPIP} with sparsity-based processing.}} & \multirow{3}{*}{Doppler} & \multirow{5}{*}{\parbox[t]{4cm}{Accuracy depends on grid resolution (meshing).\\ High computational cost.\\ Sensitive to incorrect sparsity assumption.}} \\ \cline{2-3}
 & \cite{sui2015sparse} & 2015 &  &  &  \\ \cline{2-3}
 & \cite{s18041249} & 2018 &  &  &  \\ \cline{2-5}
 & \cite{quan2018range} & 2018 & \parbox[t]{5.3cm}{Carrier frequency hopping and \gls{PRF}-jitter with sparsity-based processing.} & \multirow{2}{*}{Range-Doppler} &  \\ \cline{2-4}
 & \cite{li2021phase} & 2021 & \parbox[t]{5.3cm}{Phase transformation of range-Doppler recovery using compressed sensing for frequency.} &  &  \\ \hline
\multirow{8}{*}{\begin{tabular}[c]{@{}c@{}}Precoding \\ Strategies\end{tabular}} & \cite{akhtar2009orthogonal} & 2009 & \parbox[t]{5.3cm}{Agile signal.} & \multirow{8}{*}{\parbox[t]{1.5cm}{Range}} & \multirow{8}{*}{\parbox[t]{4cm}{Effectiveness depends on proper waveform design.\\ More predictable: risk of jammers exploiting the coding pattern.\\ Moderate computational complexity.}} \\ \cline{2-5}
 & \cite{Lei2012ARE} & 2012 & \parbox[t]{5.3cm}{Use of full-rate orthogonal pulse block design.} &  &  \\ \cline{2-4}
 & \cite{li2014frequency} & 2014 & \parbox[t]{5.3cm}{Use of frequency-agility and subband synthesis.} &  &  \\ \cline{2-4}
 & \cite{abdalla2016eccm} & 2016 & \parbox[t]{5.3cm}{Use of orthogonal designs in a netted radar system leveraging signal fusion.} &  &  \\ \cline{2-5}
 & \cite{tang2020high} & 2020 & \multirow{3}{*}{\parbox[t]{5.3cm}{Use of (group, azimuth, and element-pulse) phase coding techniques.}} & \multirow{4}{*}{Range-Doppler} &  \\ \cline{2-3}
 & \cite{chen2024deceptive} & 2024 &  &  &  \\ \cline{2-3}
 & \cite{yu2023mainbeam} & 2024 &  &  &  \\ \cline{2-4}
 & \cite{li2023random} & 2023 & \parbox[t]{5.3cm}{Combination of frequency agility and coding diversity.} &  &  \\ \hline
\end{tabular}
\end{table*}


==> manuscript_sections/taxonomy/table_detection_general.tex <==
\setlength{\arrayrulewidth}{0.1mm} % optional: adjust the thickness of table borders
\renewcommand{\arraystretch}{1.45}  % optional: adjust row height


\begin{table*}[htp]
\small
\caption{Overview of decision-making approaches for the detection/discrimination of radar deception jamming (see~\Cref{sec:detection}).}\label{table:jamming_discrimination}
\begin{tabular}{|>{\centering\arraybackslash}m{2.2cm}|>{\centering\arraybackslash}m{0.65cm}|>{\centering\arraybackslash}m{.6cm}|>{\centering\arraybackslash}m{2.2cm}|>{\centering\arraybackslash}m{3cm}|>{\centering\arraybackslash}m{1.5cm}|>{\centering\arraybackslash}m{4.8cm}|}
\hline
\rowcolor{blue!10}
\textbf{Discrimination Methodology} & \textbf{Ref.} & \textbf{Year} & \textbf{Statistics / Input Data} & \textbf{Key Technique / Architecture} & \textbf{Deception Domain
%\footnote{A line indicates the work does not specify the deception domain.}
} & \textbf{Challenges}\\ 
%A single line indicates the work does not specify the deception domain.
%Single line indicates the work does not specify deception domain. --> shorter but not correct gramatically???
%Original footnote by shuo: A single lines indicates that the work is general for jamming signals or does not mention the specific jamming-attack domain it focuses on.
\hline

\multirow{8}{*}{\begin{tabular}[c]{@{}c@{}}Hypothesis \\ Testing: GLRT\end{tabular}}
    &\cite{4203039} & 2007 & \multirow{8}{*}{\parbox[t]{1.85cm}{\centering Likelihood Ratio}} & \multirow{4}{2.2cm}{Conic rejection} & --------- & \multirow{8}{*}{\parbox[t]{4.8cm}{$\bullet$ Need for knowledge of signal statistics.\\ $\bullet$ Threshold selection.\\ $\bullet$ Sensitivity to parameter estimation.}} \\
    %\multirow{6}{*}{\parbox[t]{4cm}{$\bullet$ Coherence breaks with agile waveforms, leading to high sidelobe patterns.\\$\bullet$ Highly vulnerable, cannot handle agile deception attacks.}}
\cline{2-3}
    & \cite{4472184} & 2008 & & & & \\
\cline{2-3}
    & \cite{hao2012adaptive} & 2012 & & & & \\
\cline{2-3}\cline{6-6}
    & \cite{li2017adaptive} & 2017 & & & Range-Doppler & \\
\cline{2-3}\cline{5-5}\cline{6-6}
    & \cite{huang2013novel}\footnote{Polarimetric processing for deception jamming discrimination was first proposed in~\cite{huang2013novel}, but the work lacked a defined decision-making approach.}  & 2013 & &\multirow{3}{*}{\parbox[t]{2.2cm}{\centering Polarimetric radar system}} & ---------& \\

    %\multirow{2}{*}{\parbox[t]{1.85cm}{\centering Frequency response}} 

    
    % original footnote set by shuo: The novel idea for discriminating the deception signal with polarimetric processing was proposed in \cite{huang2013novel}, where great visualization in sinclair-scattering-matrix space was presented. They provided no certain decision-making approach though.
    \cline{2-3}\cline{6-6}
    & \cite{yu2019polarimetric} & 2019 & & & \multirow{2}{*}{\parbox[t]{1.5cm}{\centering Range}} & \\
    \cline{2-3}

    %\multirow{2}{*}{\parbox[t]{1.85cm}{\centering Frequency response}} 
    & \cite{zhang2023detection} & 2023 & & & & \\
\cline{2-3}\cline{5-5}\cline{6-6}
    & \cite{7827908} & 2017 & &Phase noise examination & Doppler & \\
\hline
% \multirow{5}{1.85cm}{Range}
\multirow{4}{*}{\begin{tabular}[c]{@{}c@{}}Self-Defined \\ Test\end{tabular}}
    & \cite{shuangcai2011algorithm} & 2011 & Phase variance & Signal extraction and sorting & Range-Doppler & \multirow{5}{5cm}{$\bullet$ Need for knowledge of signal model.\\ $\bullet$ Manual threshold selection.\\ $\bullet$ Limited generalization across radar systems and jamming types.} \\
\cline{2-5}\cline{6-6}
    & \cite{wang_2019} & 2019 & Signal power & Four-channel monopulse radar & --------- & \\
\cline{2-5}\cline{6-6}
    & \cite{guo2019improved} & 2019 & Fitting residual & Bistatic radar system & \multirow{2}{*}{\parbox[t]{1.5cm}{\centering Range}} & \\
\cline{2-5}
    & \cite{liu2021unsupervised} & 2021 & Spectrum moments and HS score & Clustering analysis &  & \\
\hline
\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Bayesian \\ Decision\end{tabular}}
    & \cite{zhou2021feature} & 2021 & Posterior probability & Multiple-feature fusion & --------- & \multirow{1}{5cm}{$\bullet$ Need for effective feature selection.\\ $\bullet$ High computational complexity.\\ $\bullet$ Sensitive to low SNR.}\\
&&&&&&\\
\cline{1-5}\cline{7-7}
\multirow{7}{*}{\begin{tabular}[c]{@{}c@{}}ML-Based \\ \footnotesize{(See Section~\ref{sec:challenge_future}} \\ \footnotesize{for strategies using}\\\footnotesize{ Transformer-based}\\\footnotesize{models)}\end{tabular}}

    & \cite{luo2021semi} & 2011 & Received time sequence & Deep belief network with pretraining &  & \multirow{7}{5cm}{$\bullet$ Choice of processing domain and transformation method.\\ $\bullet$ Need for large amount of training data.\\ $\bullet$ Risk of overfitting to simulated environment.} \\
\cline{2-5}\cline{6-6}
    &\cite{lv2021radar} & 2021 & Time–frequency spectrogram & CNN with transfer learning & \multirow{2}{*}{\parbox[t]{1.5cm}{\centering Jamming Classifier}} & \\
\cline{2-5}
    &\cite{kong2022active} & 2022 & Time–frequency and range-Doppler spectrogram & CNN with attention & &\\
\cline{2-5}\cline{6-6}
    &\cite{bouzabia2022deep} & 2022 & Choi–Williams
distribution & CNN-based & --------- &\\
\cline{2-5}\cline{6-6}
    &\cite{wang2023application} & 2023 & Received time sequence & WSN-based &\multirow{3}{*}{\parbox[t]{1.5cm}{\centering Jamming Classifier}}&\\
\cline{2-5}
    %&\cite{peng2023positive} & 2023 & \multirow{2}{1.85cm}{Frequency response} & \multirow{2}{4cm}{CNN and LSTM-based} & &\\
    &\cite{peng2023positive} & 2023 &\multirow{2}{*}{\parbox[t]{1.85cm}{\centering Frequency response}} & \multirow{2}{3cm}{\parbox[t]{3cm}{\centering CNN and LSTM-based}} & &\\
\cline{2-3}
    &\cite{wenbin2024method} & 2024 & & & &\\
    
\hline
\end{tabular}
\end{table*}
%\multirow{2}{*}{\parbox[t]{1.85cm}{\centering CNN and LSTM-based}}
 %\multirow{2}{4cm}{CNN and LSTM-based}
